Dream to Remember: Continual Steering of Generalist Robot Policies with World Models

Generalist robot policies are trained with imitation learning and are bounded by the quality and coverage of their demonstrations. Reinforcement learning can improve and extend them, either by fine-tuning the policy weights or by training a small module to steer the input noise of a frozen generative policy. When tasks arrive sequentially, both approaches suffer from catastrophic forgetting. Fine-tuning on a task degrades prior tasks, and steering only shifts forgetting to the shared steering module. We propose Dream to Remember (D2R), which continually steers a frozen generalist policy toward new tasks, while retaining its earlier skills. As the steering module learns a new task, a frozen pretrained world model rehearses prior tasks through imagined rollouts, anchoring the module to its earlier behavior without a replay buffer or new data. When the world model is faithful enough, D2R learns the new task entirely in imagination. Otherwise, it learns the task in the environment while using the world model only to rehearse prior tasks. On CALVIN, D2R improves eight tasks in sequence entirely in imagination, raising average success from 63.7% to 74.8%, while LoRA fine-tuning on the same sequence drops it to 11.7%. With a frozen off-the-shelf generalist policy and world model, $\pi_0$ and A2World, D2R learns unseen LIBERO-90 tasks in the environment while keeping $\pi_0$'s performance on the LIBERO suites it was fine-tuned on, even though the world model is not accurate enough for policy optimization. Finally, on a real Franka robot, D2R improves three tasks in sequence entirely in imagination while retaining the earlier improvements.

==> results/libero_suite_retention_data.tex <==
% Data and plot styles shared by results/libero_suite_retention_avg.tex (main text)
% and results/libero_maintaining_base_suites.tex (appendix, per suite).
% Required in the preamble:
% \usepackage{pgfplots}
% \pgfplotsset{compat=1.18}
% \usepgfplotslibrary{groupplots}

% ========================================================
% Success rates in percent
% Columns: stage, D2R-Imagined, D2R-Cache Real, D2R-No KL
%
% Stage order:
% 0: 0_close_drawer
% 1: 7_open_drawer
% 2: 9_put_bowl
% 3: 10_put_bowl
% 4: 56_pick_butter
% 5: 57_pick_creame
% 6: 20_turn_on_stove
% 7: 35_open_microwave
% ========================================================

\pgfplotstableread{
stage imagined real  nokl
0     96.67    96.67  5.33
1     98.00    97.33  81.33
2     96.67    97.00  67.00
3     98.33    96.67  60.33
4     97.00    96.33  62.00
5     97.67    97.33  73.67
6     96.33    96.33  85.67
7     97.00    96.67  77.00
}\spatialdata

\pgfplotstableread{
stage imagined real  nokl
0     96.67    95.33  30.67
1     94.67    96.67  58.67
2     95.67    96.00  75.67
3     95.33    95.67  57.00
4     95.67    95.67  57.33
5     96.67    96.67  64.67
6     97.33    95.33  72.67
7     95.67    97.33  79.00
}\goaldata

\pgfplotstableread{
stage imagined real  nokl
0     98.67    98.67  66.67
1     98.00    99.00  85.00
2     98.67    99.00  49.00
3     99.00    99.00  65.00
4     98.00    98.67  89.33
5     99.67    99.00  76.00
6     99.00    99.00  82.33
7     99.33    99.33  71.33
}\objectdata

\pgfplotstableread{
stage imagined real  nokl
0     88.00    87.67  1.33
1     89.33    87.00  30.67
2     86.33    85.67  62.00
3     87.67    87.67  33.00
4     90.00    85.33  51.33
5     89.67    86.67  33.67
6     89.00    88.67  47.33
7     88.67    88.67  37.67
}\longdata

% Reported averages across the four suites
\pgfplotstableread{
stage imagined real  nokl
0     95.00    94.59  26.00
1     95.00    95.00  63.92
2     94.34    94.42  63.42
3     95.08    94.75  53.83
4     95.17    94.00  65.00
5     95.92    94.92  62.00
6     95.42    94.83  72.00
7     95.17    95.50  66.25
}\averagedata

% ========================================================
% PI0 baselines, in percent
% ========================================================
\def\piSpatial{96.66}
\def\piGoal{94.33}
\def\piObject{97.66}
\def\piLong{90.33}
\def\piAverage{94.75}

\input{results/method_styles}


==> results/method_styles.tex <==
% Shared colors and plot styles for every method, used by all result figures.
% Rule: one color per method across the paper. Real data / real rollouts share the
% cached-rollouts color, imagined data shares the D2R color.
% Hex values mirror figures/plot_libero_memory.py (validated for colorblind separation).
% gray = frozen base / real data, warm = baselines (amber DSRL, red LoRA), blue family = ours (light = cached, dark = D2R)
\definecolor{basecolor}{HTML}{8c8c8c}
\definecolor{dsrlcolor}{HTML}{eda100}
\definecolor{loracolor}{HTML}{e34948}
\definecolor{cachedcolor}{HTML}{9cc3ec}
\definecolor{d2rcolor}{HTML}{1f5fb4}
\definecolor{realcolor}{HTML}{3d3d3d} % real data, not a method
\definecolor{imaginedcolor}{HTML}{4a3aa7} % world-model (imagined) data, not a method
\pgfplotsset{
    base bar/.style={fill=basecolor, draw=basecolor!70!black},
    dsrl bar/.style={fill=dsrlcolor, draw=dsrlcolor!70!black},
    lora bar/.style={fill=loracolor, draw=loracolor!70!black},
    cached bar/.style={fill=cachedcolor, draw=cachedcolor!70!black},
    d2r bar/.style={fill=d2rcolor, draw=d2rcolor!60!black},
    real bar/.style={fill=realcolor, draw=realcolor!70!black},
    imagined bar/.style={fill=imaginedcolor, draw=imaginedcolor!70!black},
    base curve/.style={color=basecolor!85!black, line width=1.1pt, dash pattern=on 4pt off 2.5pt, mark=none},
    dsrl curve/.style={color=dsrlcolor!85!black, thick, mark=triangle*, mark size=1.6pt, mark options={fill=white}},
    lora curve/.style={color=loracolor!85!black, thick, mark=diamond*, mark size=1.6pt, mark options={fill=white}},
    cached curve/.style={color=cachedcolor!85!black, thick, mark=*, mark size=1.4pt, mark options={fill=white}},
    d2r curve/.style={color=d2rcolor!80!black, thick, mark=square*, mark size=1.4pt, mark options={fill=white}},
    % legacy names used by older figure files
    imagined curve/.style={d2r curve},
    real curve/.style={cached curve},
    nokl curve/.style={dsrl curve},
}

